Can occupant behaviors affect urban energy planning? Distributed stochastic optimization for energy communities

To meet carbon emission reduction goals in line with the Paris agreement, planning resilient and sustainable energy systems has never been more important. In the building sector, particularly, strategic urban energy planning engenders large optimization problems across multiple spatiotemporal scales leading to necessary system scope simplifications. This has resulted in disconnected system scales, namely, building occupants and smart-city energy networks. This paper intends on bridging these disjointed scales to secure both resilient and more energy-efficient urban planning thanks to a holistic approach. The intent is to assess the aggregated impact of user behavior stochasticities on optimal urban energy planning. To this end, a stochastic energy community sizing and operation problem is designed, encompassing multi-level utilities founded on energy hub concepts for improved energy and carbon emission efficiencies. To secure the scalability of our approach, an organic spatial problem distribution suitable for field deployment is put forth, validated by a proof of concept. Uncertainty factors affecting urban energy planning are particularly examined through a local sensitivity analysis, namely, economic, climate, and occupant-behavior uncertainties. Founded on historical measurements a typical Dutch energy community composed of 41 residential buildings is designed. Results disclose a fast-converging distributed stochastic problem, where boilers are showcased as the preferred heating utility, and distributed renewable energy and storage systems were identified as unprofitable for the community. Occupant behavior was particularly exposed as the leading uncertainty factor impacting energy community planning. This demonstrates the relevance and value of our approach in connecting occupants to cities for improved, and more resilient, urban energy planning strategies.

==> manuscript/src/sections/application.tex <==
\section{Applications and Outlooks}\label{sect_app}

This works opens the door to..

==> manuscript/src/sections/elsevierGuide.tex <==
\section{The Elsevier article class}

\paragraph{Installation} If the document class \emph{elsarticle} is not available on your computer, you can download and install the system package \emph{texlive-publishers} (Linux) or install the \LaTeX\ package \emph{elsarticle} using the package manager of your \TeX\ installation, which is typically \TeX\ Live or Mik\TeX.

\paragraph{Usage} Once the package is properly installed, you can use the document class \emph{elsarticle} to create a manuscript. Please make sure that your manuscript follows the guidelines in the Guide for Authors of the relevant journal. It is not necessary to typeset your manuscript in exactly the same way as an article, unless you are submitting to a camera-ready copy (CRC) journal.

\paragraph{Functionality} The Elsevier article class is based on the standard article class and supports almost all of the functionality of that class. In addition, it features commands and options to format the
\begin{itemize}
\item document style
\item baselineskip
\item front matter
\item keywords and MSC codes
\item theorems, definitions and proofs
\item lables of enumerations
\item citation style and labeling.
\end{itemize}

\section{Front matter}

The author names and affiliations could be formatted in two ways:
\begin{enumerate}[(1)]
\item Group the authors per affiliation.
\item Use footnotes to indicate the affiliations.
\end{enumerate}
See the front matter of this document for examples. You are recommended to conform your choice to the journal you are submitting to.

\section{Bibliography styles}

There are various bibliography styles available. You can select the style of your choice in the preamble of this document. These styles are Elsevier styles based on standard styles like Harvard and Vancouver. Please use Bib\TeX\ to generate your bibliography and include DOIs whenever available.

Here are two sample references: \cite{Feynman1963118,Dirac1953888}.

==> manuscript/src/sections/nomenclature_AS.tex <==





% commands for optimization model
\newcommand{\Time}{\mathcal{T}}
\newcommand{\Sce}{\mathcal{S}}

% parameters
\newcommand{\Demand}[2]{{D_{#1}{#2}}}

% variables
\newcommand{\powerTransac}[2]{x_{{#1}{#2}}}


\tablefirsthead{\toprule}
\tablehead{\midrule}
\tabletail{\midrule}
\tablelasttail{\bottomrule}
\topcaption{Nomenclature
\label{tab:nomenclature}}
\footnotesize
\begin{supertabular}{p{0.2\linewidth}p{0.65\linewidth}}
  \multicolumn{2}{l}{\textbf{Sets}}\\\midrule
  $\Time$ & Set of time steps $t$\\
  $\Sce$ & Set of scenarios $s$\\

  \midrule\multicolumn{2}{l}{\textbf{Parameters}} \\\midrule
  $\Demand{s,t}{}$ & Electricity load scenario $s \in \Sce$ for period
  $t \in \Time$ [kWh]
  \\
  \midrule\multicolumn{2}{l}{\textbf{Variables}} \\\midrule
  $\powerTransac{s,t}{+} \in \mathbb{R}^{+}$ & Electricity to be bought from the
  electricity retailer for scenario $s \in \Sce$ and period $t \in \Time$ [kWh]
  \\
\end{supertabular}
\normalsize


==> manuscript/src/tables/hierarchy_charac.tex <==
\begin{tabular}{lllccc}
\toprule
  & \multicolumn{2}{l}{Characteristics}  &  Spatial & Temporal & Spatiotemporal \\
\midrule
  Case Study 1 & n       & [\#] & 50  & 37 & 50 \\
               & m       & [\#] & 192 & 24 & 50 \\
               & horizon & [hours] & 1  & 24 & 24 \\
  \\
  Case Study 2 & n       & [\#] & 50  & 37 & 50 \\
               & m       & [\#] & 173 & 24 & 50 \\
               & horizon & [hours] & 1  & 24 & 24 \\
\bottomrule
\end{tabular}
